A Variational Approach to Privacy and Fairness

In this article, we propose a new variational approach to learn private and/or fair representations. This approach is based on the Lagrangians of a new formulation of the privacy and fairness optimization problems that we propose. In this formulation, we aim to generate representations of the data that keep a prescribed level of the relevant information that is not shared by the private or sensitive data, while minimizing the remaining information they keep. The proposed approach (i) exhibits the similarities of the privacy and fairness problems, (ii) allows us to control the trade-off between utility and privacy or fairness through the Lagrange multiplier parameter, and (iii) can be comfortably incorporated to common representation learning algorithms such as the VAE, the $\beta$-VAE, the VIB, or the nonlinear IB.

==> ITW 2021 - A Variational Approach to Privacy and Fairness/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Color codes for comments
\definecolor{orange}{rgb}{1,0.4,0.0}
\newcommand{\rt}[1]{\textcolor{red}{{#1}}}
\newcommand{\ms}[1]{\textcolor{olive}{{#1}}}
\newcommand{\gb}[1]{\textcolor{blue}{{#1}}}
\newcommand{\brg}[1]{\textcolor{orange}{{#1}}}

%% KL divergence command
% Usage: \KL{f}{g} or \KL[\bigg]{f}{g}
\DeclarePairedDelimiterXPP{\KL}[2]{D_\textnormal{KL}}{(}{)}{}{%
#1\:\delimsize\|\:#2% 
}

%% Probability with optional conditioning
% Usage: \Prob{A \given B} or \Prob{A}
\DeclarePairedDelimiterXPP\Prob[1]{\mathbb{P}}{\lbrace}{\rbrace}{}{
\newcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}


%% L-norm
% Usage: \lnorm{x}{2} -> ||x||_2
\DeclarePairedDelimiterXPP{\lnorm}[2]{}{\lVert}{\rVert}{_{#2}}{#1}

%% Shortcuts for Algorithm, Expectation, and Real numbers
\newcommand{\bA}{\ensuremath{\mathbb{A}}}
\newcommand{\bE}{\ensuremath{\mathbb{E}}}
\newcommand{\bR}{\ensuremath{\mathbb{R}}}
\newcommand{\bN}{\ensuremath{\mathbb{N}}}
\newcommand{\bP}{\ensuremath{\mathbb{P}}}
\newcommand{\bI}{\ensuremath{\mathbbm{1}}}

%% Shortcuts for calligraphic S, T, W, X, Y, and Z
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\cW}{\ensuremath{\mathcal{W}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}

%% Shortcut for stacking something in a math equation (e.g., in a '=')
% Usage: \stack{(a)}{=}
\newcommand{\stack}[2]{\stackrel{\mathclap{(#1)}}{#2}}

%% Theorem style and definitions of different theorem-like statements
\newtheoremstyle{mytheoremstyle} % name
    {\topsep}                    % Space above
    {\topsep}                    % Space below
    {\itshape}                   % Body font
    {}                           % Indent amount
    {\bf}                        % Theorem head font
    {.}                          % Punctuation after theorem head
    {.5em}                       % Space after theorem head
    {}  % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{mytheoremstyle}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}


==> ITW 2021 - A Variational Approach to Privacy and Fairness/packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Beautiful mathematics
\usepackage{amsmath, amsthm, amssymb, amsfonts} 
\usepackage{nicefrac}
\usepackage{mathtools}
\usepackage{bm, bbm}
\usepackage{thm-restate}
\usepackage[scr=boondoxo,scrscaled=1.05]{mathalfa}

%% References in the correct format 
%\usepackage[square,numbers]{natbib}
\def\bibfont{\footnotesize} % fix to have the same font size as without natbib
\usepackage{cite}

%% Floats and tables
\usepackage{subfig}
\usepackage{booktabs}                                  

%% Enumerate nicely 
\usepackage{enumitem}

%% Different color comments and commenting large parts of the text
\usepackage{xcolor}
\usepackage{comment}

%% Hyper references
\usepackage{hyperref}
\usepackage{url}

%% Appendix package
%\usepackage{appendix}

%% Random text to test spacing 
\usepackage{blindtext}

